Secure State Estimation and Control for Cyber Security of AC Microgrids

A timely, accurate, and secure dynamic state estimation is needed for reliable monitoring and efficient control of microgrids. The synchrophasor technology enables us to obtain synchronized measurements in real-time and to develop dynamic state estimators for real-time monitoring and control of microgrids. In this study, we consider an AC microgrid comprising several synchronous generators and inverter-interface power supplies, and focus on securely estimating the dynamic states of the microgrid from a set of corrupted data. We propose a dynamic state estimator which enables the microgrid operator to reconstruct the dynamic states of the microgrid from a set of corrupted data. Finally, we consider an AC microgrid with the same topology as the IEEE 33-bus distribution system, and numerically show that the proposed secure estimation algorithm can accurately reconstruct the attack signals.

==> citepaperaa.tex <==
[1] M. Ili´c and S. Liu, Hierarchical Power Systems Control: Its Value in a
Changing Industry. Springer, 1996.

P. Kundur, et al., "Definition and classification of power system stability IEEE/CIGRE joint task force on stability terms and definitions," in IEEE Transactions on Power Systems, vol. 19, no. 3, pp. 1387-1401, Aug. 2004.

F. C. Schweppe and J. Wildes, "Power System Static-State Estimation, Part I: Exact Model," in IEEE Transactions on Power Apparatus and Systems, vol. PAS-89, no. 1, pp. 120-125, Jan. 1970.

A. Abur and A. G. Exp´osito, Power System State Estimation: Theory
and Application. Marcel Dekker, Inc., 2004.

--------------------------------------------
5
H. Modir and R. A. Schlueter, "A Dynamic State Estimator for Dynamic Security Assessment," in IEEE Transactions on Power Apparatus and Systems, vol. PAS-100, no. 11, pp. 4644-4652, Nov. 1981.

6
A. P. S. Meliopoulos et al., "Dynamic State Estimation-Based Protection: Status and Promise," in IEEE Transactions on Power Delivery, vol. 32, no. 1, pp. 320-330, Feb. 2017.

---------------------------------------------
11

V. Terzija et al., "Wide-Area Monitoring, Protection, and Control of Future Electric Power Networks," in Proceedings of the IEEE, vol. 99, no. 1, pp. 80-93, Jan. 2011.

----------------------------------------------
